Adaptive sequential Monte Carlo by means of mixture of experts

Appropriately designing the proposal kernel of particle filters is an issue of significant importance, since a bad choice may lead to deterioration of the particle sample and, consequently, waste of computational power. In this paper we introduce a novel algorithm adaptively approximating the so-called optimal proposal kernel by a mixture of integrated curved exponential distributions with logistic weights. This family of distributions, referred to as mixtures of experts, is broad enough to be used in the presence of multi-modality or strongly skewed distributions. The mixtures are fitted, via online-EM methods, to the optimal kernel through minimisation of the Kullback-Leibler divergence between the auxiliary target and instrumental distributions of the particle filter. At each iteration of the particle filter, the algorithm is required to solve only a single optimisation problem for the whole particle sample, yielding an algorithm with only linear complexity. In addition, we illustrate in a simulation study how the method can be successfully applied to optimal filtering in nonlinear state-space models.

==> sections/experts_macros.tex <==
\usepackage{graphicx}
\usepackage{amsmath,amssymb,bbm}
\usepackage{ifthen}
\usepackage{twoopt}
\usepackage{color}
\usepackage{xargs}
%\usepackage{showlabels}
%\usepackage[notref,notcite,color]{showkeys} % No keys in the text for the refs and cites


%%%%%%%%%%%%%%%%%%%%%%%%
%
% Jimmy's commands, in ALPHABETIC order....
%
%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\globmax}{\bar{\boldsymbol{\theta}}}
\newcommand{\jvect}[1]{\mathbf{#1}}
\newcommand{\jvecth}[1]{\hat{\mathbf{#1}}}
\newcommand{\meanfd}[1]{\mathbf{h}^N(#1)}
\newcommandx\n[1][1=]{
\ifthenelse{\equal{#1}{}}
{N}
{N_{#1}}
}
\newcommand{\nablapar}{\nabla_{\hspace{-0.4mm} \boldsymbol{\theta}}}
\newcommand{\noise}[1]{\boldsymbol{\xi}_{#1}}
\newcommand{\normconst}[1]{\hat{c}_{#1}}
\newcommandx\param[1][1=]{
\ifthenelse{\equal{#1}{}}
{\boldsymbol{\theta}}
{\boldsymbol{\theta}_{#1}}
}
\newcommand{\pset}{\boldsymbol{\Pi}}
\newcommand{\pstat}[2]{
\ifthenelse{\equal{#1}{}}
{\bar{\mathbf{p}}^N(#2)}
{\bar{p}^N_{#1}(#2)}
}
%\newcommand{\pstatest}[2]{
%\ifthenelse{\equal{#1}{}}
%{\hat{\bar{\mathbf{p}}}(#2)}
%{\hat{\bar{p}}_{#1}(#2)}
%}
%\newcommand{\pstatest}[2]{
%\ifthenelse{\equal{#1}{}}
%{\check{\mathbf{p}}(#2)}
%{\check{\mathbf{p}}_{#1}(#2)}
%}
%\newcommand{\pstatest}[2]{
%\ifthenelse{\equal{#1}{}}
%{\bar{\mathbf{p}}^{N_{\ell}}(#2)}
%{\bar{p}_{#1}^{N_{\ell}}(#2)}
%}
\newcommand{\pstatest}[2]{
\ifthenelse{\equal{#1}{}}
{\tilde{\mathbf{p}}^N(#2)}
{\tilde{p}^N_{#1}(#2)}
}
\newcommand{\sset}{\boldsymbol{\Sigma}}
\newcommand{\step}[1]{\lambda_{#1}}
%\newcommand{\sstatest}{\hat{\bar{\jvect{s}}}}
%\newcommand{\sstatest}{\check{\jvect{s}}}
%\newcommand{\sstatest}{\bar{\bar{\jvect{s}}}}
%\newcommand{\sstatest}{\bar{\jvect{s}}^{N_{\ell}}}
\newcommand{\sstatest}{\tilde{\jvect{s}}^N}
\newcommandx\sumwgts[2][1=]{
\ifthenelse{\equal{#1}{}}
{\tilde{\Omega}_{#2}}
{\tilde{\Omega}_{#2}^{(#1)}}
}
\newcommand{\trans}{\intercal}
\newcommand{\tstat}{\bar{\mathbf{t}}^N}
\newcommand{\vstat}{\bar{\mathbf{v}}^N}








% General maths
%\newcommand{\rightdefine}{=:}

% Laws
\newcommand{\esp}{\operatorname{\mathbb E}}
\newcommand{\prob}{\operatorname{\mathbb P}}
\newcommand{\var}{\operatorname{\mathbb V}}
\newcommand{\indic}{\mathbbm 1}

% Sets
\newcommand{\rset}{\ensuremath{\mathbb{R}}}
\newcommand{\nset}{\ensuremath{\mathbb{N}}}
\newcommand{\lone}{\ensuremath{\mathsf{L}^1}}
%\newcommand{\ltwo}{\ensuremath{\mathsf{L}^2}}
%\newcommand{\lp}{\ensuremath{\mathrm{L}^p}}

% Distributions
%\newcommand{\cauchy}{\ensuremath{\operatorname{C}}}
%\newcommand{\lognorm}{\ensuremath{\operatorname{LN}}}
%\newcommand{\dirich}{\ensuremath{\operatorname{Dir}}}
%\newcommand{\negexp}{\ensuremath{\operatorname{Exp}}}
%\newcommand{\gam}{\ensuremath{\operatorname{Ga}}}
%\newcommand{\invgam}{\ensuremath{\operatorname{IG}}}
\newcommand{\unif}{\ensuremath{\operatorname{U}}}
%%\newcommand{\betad}{\ensuremath{\operatorname{Be}}}
%\newcommand{\poiss}{\ensuremath{\operatorname{Pn}}}
\newcommand{\mult}{\ensuremath{\operatorname{Mult}}}


% Model components
% HMM representation
\newcommand{\Q}{\ensuremath{Q}}
\newcommand{\q}{\ensuremath{q}}
%14 \newcommand{\Xinit}{\ensuremath{\chi}}
%\newcommand{\Xstat}{\ensuremath{\pi}}
%\newcommand{\Xcard}{\ensuremath{r}}
%\newcommand{\order}{\ensuremath{r}}
\newcommand{\G}{\ensuremath{G}}
\newcommand{\g}{\ensuremath{g}}
%%%\newcommand{\Ycard}{\ensuremath{s}}


%%%%%%%%%%%%%%%
% HMM notations
% Hidden states and observations
\newcommand{\X}{\ensuremath{X}}
\newcommand{\x}{\ensuremath{x}}	
%14 \newcommand{\Xset}{\ensuremath{\mathsf{X}}} % 14
%14 \newcommand{\Xsigma}{\ensuremath{\mathcal{X}}} % 14
%\newcommand{\Xprocshort}{\ensuremath{\{X_k\}}}
%14 \newcommand{\Y}{\ensuremath{Y}}
%14 \newcommand{\y}{\ensuremath{y}}
%14 \newcommand{\Yset}{\ensuremath{\mathsf{Y}}}
%14 \newcommand{\Ysigma}{\ensuremath{\mathcal{Y}}}
%\newcommand{\Yprocshort}{\ensuremath{\{Y_k\}}}
%\newcommand{\Yprocone}{\ensuremath{\{Y_k\}_{k\geq 1}}} % for order chapter
%\newcommand{\XYchain}{\ensuremath{\{X_k,Y_k\}_{k\geq 0}}}
%\newcommand{\XYchainshort}{\ensuremath{\{X_k,Y_k\}}}
%\newcommand{\XYprocshort}{\ensuremath{\{X_k,Y_k\}}}
%\newcommand{\chunk}[4][]{\ensuremath{{#2\optexp{#1}_{#3:#4}}}}



% Delimiters
%\newcommand{\llb}{[\![} %\newcommand{\llb}{\llbracket}
%\newcommand{\rrb}{]\!]} %\newcommand{\rrb}{\rrbracket}
%\newcommand{\interN}[2]{\ensuremath{[\![#1, #2]\!]}}	% Integer interval, handmade
%\newcommand{\interN}[2]{\ensuremath{\llbracket #1, #2\rrbracket}}	% Integer interval, package stmaryrd
%\newcommand{\interN}[2]{\ensuremath{\{#1, \ldots, #2\}}} % Integer interval, explicit version
%\newcommand{\fraction}[1]{\left\langle#1\right\rangle}
%\newcommand{\fractionN}[1]{\langle#1\rangle}
%\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
%\newcommand{\floorN}[1]{\lfloor#1\rfloor}


% Fractional parts
\newcommand{\partfrac}[1]{\left\langle #1 \right\rangle}
%\newcommand{\partent}[1]{\left \lfloor #1 \right \rfloor}



% \newcommand{\aslim}{\ensuremath{\stackrel{\text{a.s.}}{\longrightarrow}}}


%%%%%%%%%%%%%%%%%%%%
% Particle filtering
% Estimators
\newcommand{\NISE}[4][]{\ensuremath{\tilde{#2}^{\scriptstyle \mathrm{EP}}_{\ifopt{#1}{#1,}#4}\left(#3 \right)}}
\newcommand{\ISE}[4][]{\ensuremath{\widehat{#2}^{\scriptstyle  \mathrm{EP}}_{\ifopt{#1}{#1,}#4} \left(#3 \right)}}
\newcommand{\SIRE}[4][]{\ensuremath{\hat{#2}^{\scriptstyle  \mathrm{EPR}}_{\ifopt{#1}{#1,}#4} \left(#3 \right)}}
%\newcommand{\MCE}[3]{\ensuremath{\hat{#1}^{\scriptstyle  \mathrm{MC}}_{#3} \left(#2 \right)}}
%%%

% IS, SISR, ...
% Importance sampling dist.
\newcommand{\XinitIS}{\ensuremath{\rho_0}}
\newcommand{\ISD}[1]{\ensuremath{\rho_{0:#1}}}
% Particle approximation to TAR
\newcommand{\ETAR}[1]{\ensuremath{\hat{\phi}_{0:#1|#1}}}

%%% State-space notations
% State-space representation
\newcommand{\A}{\ensuremath{A}}
\newcommand{\Afunc}{\ensuremath{a}}
\newcommand{\U}{\ensuremath{U}}
%\newcommand{\Uobs}{\ensuremath{u}}
%\newcommand{\Uprocshort}{\ensuremath{\{U_k\}}}
\newcommand{\URoot}{\ensuremath{R}}
%\newcommand{\UCov}[1][]{\URoot\optsub{#1} \URoot^t\optsub{#1}}
\newcommand{\V}{\ensuremath{V}}
%\newcommand{\Vobs}{\ensuremath{v}}
%\newcommand{\Vprocshort}{\ensuremath{\{V_k\}}}
\newcommand{\VRoot}{\ensuremath{S}}
\newcommand{\VCov}[1][]{\VRoot\optsub{#1} \VRoot^t\optsub{#1}}
\newcommand{\B}{\ensuremath{B}}
\newcommand{\Bfunc}{\ensuremath{b}}
\newcommand{\dimx}{\ensuremath{d_x}}
\newcommand{\dimy}{\ensuremath{d_y}}
\newcommand{\dimu}{\ensuremath{d_u}}
\newcommand{\dimv}{\ensuremath{d_v}}
\newcommand{\dimpsp}{p}
\newcommand{\dimpsptd}{\tilde p}

\newcommand{\Amat}{\Lambda}
\newcommand{\Bmat}{\Gamma}



%%%%%%%%%%%%%%%%%%%%%%%%%
% Kalman filter notations
%\newcommand{\projx}[3]{\ensuremath{\hat{#1}_{#2|#3}}}
%\newcommand{\filtmean}[1]{\ensuremath{\hat{X}_{#1|#1}}}
%\newcommand{\filtcov}[1]{\ensuremath{\Sigma_{#1|#1}}}
%\newcommand{\postmean}[2]{\ensuremath{\hat{X}_{#1|#2}}}
%\newcommand{\postcov}[2]{\ensuremath{\Sigma_{#1|#2}}}
%\newcommand{\I}{\ensuremath{\epsilon}}
%\newcommand{\ICov}{\ensuremath{\Gamma}}
%\newcommand{\KGP}[1]{\ensuremath{H_{#1}}}
\newcommand{\KGF}[1]{\ensuremath{K_{#1}}}
% Disturbance smoother variables
%\newcommand{\trmat}{\ensuremath{\Lambda}}
%\newcommand{\iqsm}{\ensuremath{p}}
%\newcommand{\IQsm}{\ensuremath{C}}



%%%%% Genalogical tree notations %%%%%
% Genealogic particle
%\newcommand{\genepart}[3]{\ensuremath{\xi^{\ifopt{#3}{#3,}#2}_{#1}}}
%\newcommand{\genepartN}[3]{\genepart{#1,N}{#2}{#3}}
% Ancester's index
%\newcommand{\geneind}[3]{\ensuremath{I^{\ifopt{#3}{#3,}#2}_{#1}}}
%\newcommand{\geneindN}[3]{\geneind{#1,N}{#2}{#3}}
% Sets

%\newcommand{\stsp}{{\boldsymbol{\Xi}}}
% Sets
%\newcommand{\Nst}{\mathbb{N}^*}
%%%%% APF
%\newcommand{\APF}{PFA\ }
\newcommand{\bddonX}[1]{\mathcal{B}_{\mathrm{b}}(\stsigma^{#1})}
%14 \newcommand{\define}{:=} % triangleq
\newcommand{\E}{\mathbb{E}}
\newcommand{\filt}[1]{\mathcal{F}_{#1}}
\newcommand{\filthat}[1]{\hat{\mathcal{F}}_{#1}}
\newcommand{\filttilde}[1]{\tilde{\mathcal{F}}_{#1}}
\newcommand{\fop}[2]{\Psi_{#1:#2}} % A VOIR, utilis� dans un seul lemme
\newcommand{\fstimp}[1]{\varphi_{#1}^N} % N'est pas auxinstr, est une mesure o� seul est utilis� \adj, pas \wgt ...
%14 \newcommand{\fstimpfunc}[1]{\fstimpfuncletter_{#1}}
%14 \newcommand{\fstimpfuncletter}{t}
\newcommand{\fsttarg}[1]{\alpha_{#1}^N} % N'est autre que auxtarg
%14 \newcommand{\fstwgt}[2]{{\tau}_{#1}^{N,#2}}
\newcommand{\hd}[1]{q_{#1}}
% Original: \newcommand{\hk}[1]{Q_{#1}}, changed to encompass STCO
%14 \newcommand{\hk}[1][]{Q\optsub{#1}}
\newcommand{\lb}{\epsilon_-}
%\newcommand{\lf}[1]{g_{#1}}
\newcommand{\lf}{g}
\newcommand{\Lp}[1]{\mathsf{L}^{#1}}
%\newcommand{\opt}[1]{H_{#1}}
\newcommand{\osc}{\operatorname{osc}}
\newcommand{\overpil}[1]{\raisebox{1.5ex}{ $\underrightarrow{\text{\ \scriptsize #1\ }}$ }}
%\newcommand{\Prob}{\operatorname{\mathbb{P}}}

% WARNING !
\newcommand{\partsmooth}[2]{\phi^N_{\Xinit,#1|#2}}
\newcommand{\partsmoothtilde}[2]{\tilde{\phi}^N_{\nu,#1}}%|#2}}

%\newcommand{\parttilde}[3]{\tilde{\xi}_{#1}^{N,#2}\ifopt{#3}{(#3)}}
% TODO: CHECK if \refm should call \targ
\newcommand{\refm}{\mu}
%\newcommand{\PSimpfunct}[1]{\fstimpfunc{#1}^{\mathrm{P\&S}}}
\newcommand{\sdimpfunc}[1]{\sdimpfuncletter_{#1}}
\newcommand{\sdimpfuncletter}{w}
\newcommand{\sdtarg}[1]{\beta_{#1}^N}
%\newcommand{\smooth}[2]{\phi_{\nu,#1}}%|#2}}
%\newcommand{\smooth}[1]{\phi_{\Xinit,#1}}
\newcommand{\smoothmixture}[2]{\bar{\phi}^N_{\Xinit,#1|#2}}
\newcommand{\smoothop}[1]{\Phi_{#1}}%|#2}}
\newcommand{\supnm}[2]{\left \| #2 \right \|_{#1, \infty}}
%\newcommand{\SSAPF}{SSAPF\ }
%\newcommand{\TSS}{TSSPF\ }
\newcommand{\ub}{\epsilon_+}
%\newcommand{\Xsigm}{\Xsigma}
%\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\vect}[1]{#1}
%\newcommand{\yrefm}{\lambda}
%\newcommand{\Ysigm}{\Ysigma}
%\newcommand{\wgt}[2]{\omega_{#1}^{N,#2}}
%14 \newcommand{\wgtsum}[1]{\Omega_{#1}^N}
%14 \newcommand{\wgtsumtilde}[1]{\tilde{\Omega}_{#1}^N}
%\newcommand{\wgttilde}[2]{\tilde{\omega}_{#1}^{N,#2}}



%%%%% REQUIRED FOR ASYMPTOTICS ?? %%%%%%%%%%%%%
\newcommand{\mcf}[2][]{\mathcal{F}_{#2}\optpexp{#1}}

%14 \newcommand{\PP}{\prob}
%14 \newcommand{\PE}{\esp}
%14 \newcommand{\CPE}[3][]{\esp\optsub{#1}\left[\left. #2 \, \right | #3 \right]}
%14 \newcommand{\CPP}[3][]{\prob\optsub{#1}\left(\left. #2 \, \right | #3 \right)}

%14 \newcommand{\eqdef}{\define}
\def\consistfunc{\ensuremath{\mathsf{C}}}
\def\asnormfunc{\ensuremath{\mathsf{A}}}
\def\consistweight{\ensuremath{\mathsf{W}}}
\def\stdnormfunc{\sigma}


%\newcommand{\epartset}{\ensuremath{\boldsymbol{\Xi}}}
%\newcommand{\epartsigma}{\ensuremath{\mathcal{B}(\boldsymbol{\Xi})}}
%\newcommand{\etpartset}{\ensuremath{\boldsymbol{\tilde{\Xi}}}}
%\newcommand{\etpartsigma}{\ensuremath{\mathcal{B}(\boldsymbol{\tilde{\Xi}})}}

%14 \newcommand{\epart}[2][]{\ensuremath{\xi_{#2}\optpexp{#1}}}
%14 \newcommand{\ebwght}[2]{\ensuremath{\bar{\omega}_{#1}^{#2}}}

%14 \newcommand{\etpart}[2][]{\ensuremath{\tilde{\xi}_{#2}\optpexp{#1}}}
%\newcommand{\ebpart}[2][]{\ensuremath{\bar{\xi}_{#2}\optpexp{#1}}}
%14 \newcommand{\sumweight}[2][]{\ensuremath{\Omega_{#2}\optpexp{#1}}}
%14 \newcommand{\ewght}[2][]{\ensuremath{\omega_{#2}\optpexp{#1}}}
%14 \newcommand{\etwght}[2][]{\ensuremath{\tilde{\omega}_{#2}\optpexp{#1}}}
%14 \newcommand{\ind}[2][]{\ensuremath{I_{#2}\optpexp{#1}}}
%14 \newcommand{\indTSS}[2][]{\ensuremath{J_{#2}\optpexp{#1}}}
\newcommand{\funcweight}{\ensuremath{\Phi}}
\def\LTAR{L}
\newcommand\ntimes[1]{G_{#1}}
\newcommand\ntimesres[1]{H_{#1}}
\newcommand{\1}{\indic}
\newcommand{\PVar}{\var}

%%%%%%% FEBRUARY 14 %%%%%%%%%%%%%%%%%%%%%
%%%%%%% UNIFORMIZED NOTATIONS %%%%%%%%%%%
\numberwithin{equation}{section}

% ---- Annotations ----
%\newcommand{\Note}[2]{\marginpar{\textcolor{blue}{#1} \color{red}\footnotesize{ #2}\color{black}}}
\newcommand{\Note}[2]{\footnote{\textcolor{blue}{#1} \color{red}\footnotesize{ #2}\color{black}}}
%\newcommand{\note}{\Note}
%\renewcommand{\Note}[2]{}
\newcommand{\havalook}[1]{{ \color{red} #1 }}

% ---- Lengths ----
\newcommand{\eqsp}{}
%\newcommand{\eqsp}{\;}
\newlength{\vertsepeq} \setlength{\vertsepeq}{0.5em} % Vertical equation separation in an array

% ---- Metacommand used to build commands ----
% To be used inside a command having its first argument optional and empty by default
\newcommand*{\ifopt}[2]{\ifthenelse{\equal{#1}{}}{}{#2}} % Issue nothing if the 1st argument is empty, else print the second argument
\newcommand*{\ifbothopt}[3]{\ifopt{#1}{\ifopt{#2}{#3}}}
\newcommand*{\optexp}[1]{\ifopt{#1}{^{#1}}} % Puts the argument in exponent if it is non-empty
\newcommand*{\optpexp}[1]{\ifopt{#1}{^{(#1)}}} % Puts the argument in parentheses-ed exponent if it is non-empty
\newcommand*{\optsub}[1]{\ifopt{#1}{_{#1}}} % Puts the argument in subscript if it is non-empty

% ----- General maths ----
\newcommand{\fract}[2]{#1 / (#2)} % Text frac
\newcommand{\eqdef}{:=}
\newcommand*{\equp}{\equiv} % Equality up to an irrelevant additive constant
\newcommand*{\chol}{\operatorname{chol}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand*{\extd}[1]{\overline{#1}}
%\newcommand{\ud}{\mathrm{d}}	% straight d
\newcommand{\ud}{d}
\newcommand{\mcb}[1]%
	{\ensuremath{\mathcal{F}_{\mathrm{b}}\left(#1\right)}} %Measurable bounded functions
\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\newcommand{\alg}{\mathcal{B}}
\newcommand*{\prmat}{\,}
\newcommand{\meas}{\mathcal{P}}
\newcommand{\measfunc}{\mathbb{B}}

% ---- Distributions ----
\newcommand{\normpdf}{\mathcal{N}}
\newcommand*{\normdens}[4][]{\mathcal{N}\optsub{#1}\left(#2; #3, #4\right)}
\newcommand{\bin}{\ensuremath{\operatorname{Bin}}}
\newcommand{\ber}{\ensuremath{\operatorname{Ber}}}
\newcommand{\pois}{\ensuremath{\operatorname{Pois}}}

% ----- Standard abbreviations ----
\newcommand{\wrt}{w.r.t.}
\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
\newcommand{\cf}{cf.}

% ----- State-space model -----
\newcommand{\stsp}[1][]{{\mathsf{X}\optpexp{#1}}} % State space at one time
\newcommand{\stsigma}[1][]{\ensuremath{\mathcal{X}\optpexp{#1}}}
\newcommand{\stsptd}[1][]{{\mathsf{\td{X}}\optpexp{#1}}} % State space at one time NOT SURE I NEED IT ?
\newcommand{\obsp}[1][]{{\mathsf{Y}\optpexp{#1}}} % Observation space at one time
\newcommand{\obsigma}[1][]{{\mathcal{Y}\optpexp{#1}}} % Observation space at one time
\newcommand{\xpa}{x} % Past time
\newcommand{\ypa}{y} % Past time
\newcommand{\xpr}{x'} % Present time
\newcommand{\ypr}{y'} % Present time
\newcommand{\Xinit}{\ensuremath{\chi}} % Initial distribution
\newcommand{\Xproc}{\ensuremath{\{X_k\}_{k\geq 0}}}
\newcommand{\Yproc}{\ensuremath{\{Y_k\}_{k\geq 0}}}
\newcommand{\XYproc}{\ensuremath{\{(X_k,Y_k)\}_{k\geq 0}}}
\newcommand{\Vproc}{\ensuremath{\{V_k\}_{k\geq 0}}}
\newcommand{\Uproc}{\ensuremath{\{U_k\}_{k\geq 0}}}
%\newcommand{\lhood}[2][]{\ensuremath{\mathcal{L}_{\ifopt{#1}{#1,}#2}}}	%Likelihood
\newcommand*{\lhood}[1]{\ensuremath{p_{#1}}}
%\newcommand{\post}[3][]{\ensuremath{\phi_{\ifopt{#1}{#1,}#2|#3}}} 	% Smoothing, Xinit as opt #1
\newcommand*{\post}[2]{\phi_{#1|#2}}
\newcommand{\filtpost}[2][]{\ensuremath{\phi_{\ifopt{#1}{#1,}#2}}}	% Filtering
%\newcommand{\smooth}[2]{\post[\Xinit]{#1}{#2}}
\newcommand{\TARnoi}[1]{\ensuremath{\phi_{0:#1|#1}}}
\newcommand{\TARapf}[1]{\ensuremath{\phi_{\Xinit,0:#1|#1}}}

% ----- Kernels -----
%\newcommand{\hk}[1][]{Q\optpexp{#1}}	% Transition kernel of the hidden chain
\newcommand*{\hk}{Q}
\newcommand{\hkdens}[1][]{q\optpexp{#1}}	% Transition kernel of the hidden chain
\newcommand{\ok}[1][]{G\optpexp{#1}}	% Transition kernel of the observation chain
\newcommand{\okdens}[1][]{g\optpexp{#1}}	% Transition kernel of the observation chain
\newcommand{\olik}[1][]{g\optsub{#1}}	% Local likelihood
\newcommand{\ukhmm}[1][]{\ensuremath{T\optpexp{#1}}}
\newcommand{\ukhmmdens}[1][]{\ensuremath{t\optpexp{#1}}}
%\newcommand{\uk}[1][]{L\optsub{#1}}
%\newcommand{\uk}[1]{L_{#1}}
\newcommand*{\uk}{L}
\newcommand{\ukdens}[1][]{l\optsub{#1}}
\newcommand{\uknorm}[1][]{L^\ast\optsub{#1}}
\newcommand{\uknormdens}[1][]{l^\ast\optsub{#1}}
\newcommand{\ukpath}[1][]{L_{\mathrm{p}\ifopt{#1}{,#1}}}
\newcommand{\uknormpath}[1][]{L^\ast_{\mathrm{p}\ifopt{#1}{,#1}}}
\newcommand{\prop}[1][]{R\optsub{#1}}
\newcommand{\propdens}[1][]{r\optsub{#1}}
\newcommand{\pathprop}[1]{R_{#1}^{\mathrm{p}}}
\newcommand*{\propparam}[1]{\prop_{#1}}


% ------ Limits -----
\newcommand{\dlim}{\ensuremath{\stackrel{\mathcal{D}}{\longrightarrow}}}
\newcommand{\plim}{\ensuremath{\stackrel{\mathbb{P}}{\longrightarrow}}}

% ----- Criterion ----
\newcommand{\CV}{\ensuremath{\mathrm{CV}}}
\newcommand{\CVsq}{\ensuremath{\mathrm{CV}^2}}
\newcommandx\entropy[1][1=]{
\ifthenelse{\equal{#1}{}}
{\ensuremath{\mathcal{E}}}
{\ensuremath{\mathcal{E}_{#1}}}
}

\newcommand{\ESS}{\ensuremath{\mathrm{ESS}}}

% ----- Target and proposals ----
%\newcommand{\targ}[1][]{\mu_{N\ifopt{#1}{,{#1}}}}
\newcommand{\targ}{{\tilde\mu}}
\newcommand{\src}{\mu}
% \newcommand*{\targ}{\hat\mu}
\newcommand{\propjoint}{\pi^\ast}
\newcommand{\targjoint}{\mu^\ast}
%\newcommand{\auxtarg}[1][]{\mu^{\ifasymptotic N \fi\ifopt{#1}{\ifasymptotic , \fi#1}}_{\mathrm{aux}}}
%\newcommand*{\auxtarg}{\mu^{\mathrm{aux}}}
\newcommand*{\auxtarg}{\bar{\mu}^N}

\newcommand{\prior}{\pi_0}
\newcommand{\instr}[1][]{\pi^N\ifopt{#1}{_{#1}}}
% Version with aux supersript
%\newcommand{\auxinstr}[1][]{\pi_{\ifasymptotic N \fi\ifopt{#1}{\ifasymptotic , \fi#1}}^{\mathrm{aux}}}
%\newcommand{\auxinstrparam}[1]{\pi_{\ifasymptotic N,\fi #1}^{\mathrm{aux}}}
% Version without aux superscript
%\newcommand{\auxinstr}[1][]{\pi_{\ifasymptotic N \fi\ifopt{#1}{\ifasymptotic ,
%\fi#1}}}
\newcommand{\auxinstr}[1][]{\pi^N\ifopt{#1}{#1}}
\newcommand{\auxinstrparam}[1]{\pi^N_{#1}}
\newcommand*{\mixparamvec}[1][]{\boldsymbol\theta\optexp{#1}} % Whole vector of parameters


% ----- Particles -----
% Symbols
%\newcommand*{\symp}{\xi}	% symbol for particles
%\newcommand*{\symP}{\xi}	% symbol for particles
%\newcommand*{\symW}{\Omega} % Symbol for weight
%\newcommand*{\symw}{\omega} % Symbol for weight
%\newcommand*{\symI}{I}	% Symbol for individual
\newcommand*{\symp}{{\mathbf{x}}}	% symbol for particles
\newcommand*{\symP}{{\mathbf{X}}}	% symbol for particles
\newcommand*{\symw}{\omega} % Symbol for weight
\newcommand*{\symW}{\Omega} % Symbol for weight
\newcommand*{\symi}{i}	% Symbol for individual
\newcommand*{\symI}{I}	% Symbol for individual
\newcommand*{\symj}{j}	% Symbol for component index
\newcommand*{\symJ}{J}	% Symbol for component index
\newcommand*{\symadj}{a}	% Symbol for adjustment weights
\newcommand*{\symAdj}{a}	% capital Symbol for adjustment weights
% Symbol for tildes
\newcommand*{\td}[1]{\tilde{#1}} % Either tilde or '
\newcommand*{\optim}[1]{{#1}^\ast} % optimal (not sure about this very command, beware of double superscript)
\newif\ifasymptotic
\asymptoticfalse
% Space of particles
\newcommand*{\psp}[1][]{\ensuremath{\boldsymbol{\Xi}\optsub{#1}}}		% ideally, should be mathbb of symP
\newcommand*{\psigma}{\ensuremath{\mathcal{B}(\psp)}}		% ideally, should be mathbb of symP
\newcommand*{\psptd}{\ensuremath{\boldsymbol{\td{\Xi}}}}		% ideally, should be mathbb of symP
\newcommand*{\psigmatd}{\ensuremath{\mathcal{B}(\psptd)}}
% Elements of these spaces. Ideally, should make the difference capital/small
\newcommand*{\ppa}{\symp}	% value of a past particle
\newcommand*{\ppr}{\td{\symp}} % value of a present particle
\newcommand*{\ppava}{\symP}	% r.v. \psp-valued (SUCKS, should be capitalized differently than ppa, horrible !)
\newcommand*{\pprva}{\td{\symP}} % r.v. \psptd-valued
\newcommand*{\comp}{\symj}
\newcommand*{\compva}{\symJ}
\newcommand*{\indv}{\symi}
\newcommand*{\indva}{\symI}
% Base command for all notations, to ensure coherent positioning
% of (sub|super)scripts. Takes 4 arguments:
% 1. symbol,
% 2. time -- will be parenthesized
% 3. iteration,
% 4. index -- with or without N, up to the caller
\newcommand*{\base}[4]{
	\ensuremath{%
	{#1}
	% Special case: if only #2 or #3 is set,
	\ifopt{#2#3}{^%
	{
		\ifopt{#2}{(#2)}
		\ifbothopt{#2}{#3}{,}
		\ifopt{#3}{[#3]}
	}
	}
	\ifasymptotic
	_{N\ifopt{#4}{,}#4}
	\else
	\ifopt{#4}{_{#4}}
	\fi
	}
}
% Same, but don't use the asymptotic N, ever
\newcommand*{\baseneverN}[4]{%
	{\asymptoticfalse\base{#1}{#2}{#3}{#4}} % NEVER EVER remove the outside
	% grouping parentheses, they keep \asymptoticfalse local to the command !!
}

% Environment for asymptotic analysis: all the quantities will have the added subscript N
\newenvironment{asymptotic}{\asymptotictrue}{\asymptoticfalse}
% Optional time (if one arg specified, it is time), optional iteration, mandatory index
\newcommandtwoopt*{\parti}[3][][]{\base{\symP}{#1}{#2}{#3}}
\newcommandtwoopt*{\partiva}[3][][]{\base{\symP}{#1}{#2}{#3}}
\newcommandtwoopt*{\partiextd}[3][][]{\base{\extd{\symP}}{#1}{#2}{#3}}
\newcommandtwoopt*{\wgt}[3][][]{\base{\symw}{#1}{#2}{#3}}
\newcommand*{\wgtb}[1]{\base{\bar{\symw}}{}{}{#1}}
\newcommandtwoopt*{\wgtsum}[2][][]{\base{\symW}{#1}{#2}{}}
\newcommandtwoopt*{\ind}[3][][]{\base{\symI}{#1}{#2}{#3}}
\newcommandtwoopt*{\indTSS}[3][][]{\base{J}{#1}{#2}{#3}}
% Tilde versions
\newcommandtwoopt*{\partitd}[3][][]{\base{\td{\symP}}{#1}{#2}{#3}}
\newcommandtwoopt*{\partibar}[3][][]{\base{\bar{\symP}}{#1}{#2}{#3}}
\newcommandtwoopt*{\wgttd}[3][][]{\base{\td{\symw}}{#1}{#2}{#3}}
\newcommandtwoopt*{\wgtbar}[3][][]{\base{\bar{\symw}}{#1}{#2}{#3}}
\newcommandtwoopt*{\wgtsumtd}[2][][]{\base{\td{\symW}}{#1}{#2}{}}
\newcommandtwoopt*{\wgtsumbar}[2][][]{\base{\bar{\symW}}{#1}{#2}{}}
\newcommand*{\Ntd}{M_N}
% Hat versions
\newcommandtwoopt*{\partihat}[3][][]{\base{\hat{\symP}}{#1}{#2}{#3}}
% Adjustment weights -- Typically, hjere, should get rid of \\base call
\newcommandtwoopt*{\adj}[3][][]{\base{\symadj}{#1}{#2}{#3}}
\newcommand*{\adjfunc}[1][]{\baseneverN{\symAdj}{#1}{}{}} % Do not allow iterations for now, messes up APF !
\newcommandtwoopt*{\adjfuncpath}[2][][]{\symAdj^{\mathrm{p}\ifopt{#1}{,(#1)}\ifopt{#2}{,[#2]}}}
%\newcommandtwoopt*{\adjopt}[3][][]{\base{\optim{\symadj}}{#1}{#2}{#3}}
\newcommandtwoopt*{\adjopt}[3][][]{\base{\symadj^{\ast}}{#1}{#2}{#3}}
\newcommand*{\adjfuncopt}[1][]{\baseneverN{\optim{\symAdj}}{#1}{}{}}
\newcommand*{\adjfuncoptpath}[1][]{\symAdj^{\ast \mathrm{p}\ifopt{#1}{,(#1)}}}
\newcommand*{\adjfuncPS}[1]{\adjfunc[#1]_{\mathrm{P\&S}}}
\newcommand{\wgtfunc}{w}

% ------ Divergences ----
\newcommand{\CSD}{\mathrm{CSD}}
\newcommand{\KLD}{\ensuremath{\mathrm{KLD}}}
\newcommand{\chitwo}{d_{\chi^2}}
\newcommand{\KL}{\ensuremath{d_{\mathrm{KL}}}}

% \newtheorem{theorem}{\legendTheorem}[section]
% \newtheorem{lemma}{\legendLemma}[section]
% \newtheorem{corollary}{\legendCorollary}[section]
\newtheorem{proposition}{Proposition}[section]
% \theoremstyle{definition}
% \newtheorem{definition}{\legendDefinition}[section]
% \newtheorem{example}{\legendExample}[section]
% \theoremstyle{remark}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{remark}{Remark}[section]
% \makeatletter
% \renewcommand{\ALG@name}{\legendAlgorithm}
% \makeatother

% ---- Counter for Hypothesis ----
\newcounter{hyp}
\newenvironment{hyp}[1]%
	{\refstepcounter{hyp}\it\begin{itemize}\item[{\bf(A\arabic{hyp})}] \label{hyp:#1}}%
			{\end{itemize}}
\newcommand{\refhyp}[1]{{\bf (A\ref{hyp:#1})}}



%%% MACROS FOR WORK ON EXPERTS
% Taken from macros_experts.tex


%%%% PARTICLES %%%%
\newcommand*{\wgtmean}[1][]{\mathcal{C}\optexp{#1}}	% Mean of the weights, converges to normalising factor

%%%% KERNELS %%%%
\newcommand*{\rmd}{\mathrm{d}}
\newcommand*{\propdensparam}[1]{\propdens_{#1}}
% PILOT \newcommand*{\uknorm}{L^\ast}
% PILOT \newcommand*{\uknormdens}{l^\ast}
%14 \newcommand*{\hkdens}{q}

%%%% INTEGRATED CURVED EXPONENTIAL FAMILY %%%%
%\newcommand*{\cA}{A}	% function of \curpar
\newcommand*{\cA}{a}	% function of \curpar
%\newcommand*{\cB}{B}	% function of \curpar in the scalar product
\newcommand*{\cB}{\mathbf{b}}	% function of \curpar in the scalar product
\newcommand*{\uu}{\mathbf{u}}	% variable integrated, value
\newcommand*{\uureal}{u}	% variable integrated, value
\newcommand*{\uuva}{\mathbf{U}}	% variable integrated, random variable
\newcommand*{\uurealva}{U}	% variable integrated, random variable
%\newcommand*{\uusp}{\mathbb{U}}	% space of the integrated variable
\newcommand*{\uusp}{{\boldsymbol{\Upsilon}}}	% space of the integrated variable
\newcommand*{\curvparj}[1]{{\boldsymbol\eta_{#1}}}	% parameter of the distribution
\newcommand*{\curvpar}[1][]{{\boldsymbol\eta\optsub{#1}}}	% parameter of the distribution
\newcommand*{\curvparvec}[1][]{\underline{\boldsymbol\eta}\optexp{#1}}	% vector of parameter of the components
\newcommand*{\curvparvecsp}{\mathbb{E}}
%\newcommand*{\intcurv}[3]{\rho\left(#1,#2;#3\right)}% integrated curved
\newcommand*{\intcurv}[3]{\rho(#1,#2;#3)}% integrated curved
\newcommand*{\intcurvj}[3][j]{\intcurv{#2}{#3}{\curvpar_{#1}}} % same, component j
%\newcommand*{\curv}[4]{\rho^{e}\left(#1,#2,#3;#4\right)}% extended curved
%\newcommand*{\curv}[4]{\bar{\rho}\left(#1,(#2,#3);#4\right)}% extended curved
\newcommand*{\curv}[4]{\bar{\rho}(#1,(#2,#3);#4)}% extended curved
\newcommand*{\curvj}[4][j]{\curv{#2}{#3}{#4}{\curvpar_{#1}}} % same, component j
\newcommand*{\curvsuffstat}[4]{S_{#1}\left(#2,#3,#4 \right)}  % Sufficient statistics
%\newcommand*{\curvexpestat}[2]{S_{#1}\left(#2\right)}  % Expected sufficient statistics
\newcommand*{\curvexpestat}[2]{\bar{\mathbf{s}}^N_{#1}(#2)}  % Expected
% sufficient statistics \newcommand*{\curvexpestatvec}[2]{S_{#1}\left(#2\right)}  % Expected sufficient statistics


%%%% AUXILIARY DISTRIBUTIONS %%%%
\newcommand*{\hauxtarg}[1]{\hat{\mu}^{\mathrm{aux}}_{[#1]}}

\newcommand*{\auxinstrextd}[1]{\bar{\pi}^N_{#1}}
%\newcommand*{\auxinstrextd}[1]{\pi^{e}_{#1}}
\newcommand*{\auxinstrparamdens}[1]{p_{#1}}
\newcommand*{\completelike}[1]{\auxinstrextd{#1}}
\newcommand*{\normaliselike}[1]{\mathcal{Z}_{#1}}
% PILOT \newcommand*{\:djfuncopt}{\Psi^\ast}

%%%% STATE SPACE %%%%
%\newcommand*{\stsp}{{\boldsymbol{\Xi}}}
%\newcommand*{\stsptd}{{\tilde{\boldsymbol{\Xi}}}}
\newcommand*{\dimosp}{p}
\newcommand*{\dimosptd}{p'}
%\newcommand*{\stsptd}{{\tilde{\mathsf{\symP}}}}
%\newcommand*{\xprva}{{\symP'}} % X PResent
%\newcommand*{\xpava}{\symP}			% X PAst
\newcommand*{\ds}{\ensuremath{d_s}}			% Dimension of the state space

%%%% MEASURE THEORIC %%%%%
\newcommand*{\supp}{\text{supp}}
\newcommand*{\p}{p} % density placeholder, might be $f$ instead of $p$
\newcommand*{\Expect}[2][]{\E\ifopt{#1}{_{#1}}\left[#2\right]}
\newcommand*{\Expectline}[2][]{\E\ifopt{#1}{_{#1}}[#2]}
\newcommand*{\hExpect}[2][]{\hat{\E}\ifopt{#1}{^{[#1]}}_{\auxtarg}\left[#2\right]}
\newcommand*{\Proba}[2][]{\mathbb{P}\ifopt{#1}{_{#1}}\left[#2\right]}
\newcommand*{\CProba}[2]{\left[ #1 \middle| #2\right]}
%%%% GENERAL MATHS %%%%
% PILOT \newcommand*{\N}{\mathbb{N}}
\newcommand*{\normlaw}[3][]{\mathcal{N}\optsub{#1}\left(#2, #3\right)}
\newcommand*{\vectornorm}[1]{\left\|#1\right\|}

%%%% NEWTON RAPHSON %%%%
\newcommand*{\nablaop}[1]{\nabla_{\hspace{-0.4mm} #1}}
%\newcommand{\hessian}[1]{\nabla_{\hspace{-1mm} #1} \nabla_{\hspace{-1mm} #1}^T}
\newcommand*{\hessian}[1]{\nabla^2_{\hspace{-0.4mm} #1}}
\newcommand*{\isnrdir}[1][]{\hat{\boldsymbol d}\optexp{#1}}
\newcommand*{\nrdir}[1][]{\boldsymbol d\optexp{#1}}
\newcommand*{\nrstepsize}[1][]{\tau\optsub{#1}}
\newcommand*{\sastepsize}[1][]{\lambda\optsub{#1}}

%%%% MATRICES AND VECTORS %%%
\newcommand{\trace}{\text{Tr}}
%\newcommand*{\prmat}{\cdot}
%\newcommand*{\prmat}{\,}
%\newcommand*{\prscal}[2]{\left< #1, #2 \right>}
\newcommand*{\prscal}[2]{ \tr\left({#1}^\trans #2\right)}
%\newcommand*{\diag}{\operatorname{diag}}
%\newcommand*{\chol}{\operatorname{chol}}
\newcommand*{\matsymposspace}[1]{\mathcal{M}_{s}^{+}(#1)}
\newcommand*{\matspace}[1]{\mathcal{M}(#1)}
\newcommand*{\detm}[1]{\left\vert #1\right\vert}
\newcommand*{\tr}{\mathrm{Tr}}
\newcommand*{\vnorm}[2][]{\left\| #2 \right\|\optsub{ #1}} % Norm with metric #1
\newcommand*{\mahalanobis}[3]{\delta( #1,#2,#3)} % Squared Mahalanobis distance
%\newcommand*{\mahalanobis}{3}{\euclid{#1}{#2}{#3^{-1}}^2} % alternate notation
\newcommand*{\euclid}[3][]{\vnorm[#1]{ #2 - #3}}	% Euclidian distance with metric matrix #3

%%%%% MATRIX CALCULUS %%%%
\newcommand{\dimo}{p}
\newcommand{\dpart}[2][]{\partial_{#1#2}}
\newcommand{\mati}[2]{E_{{#1 #2}}}
\newcommand{\kron}[2]{\delta_{{#1 #2}}}
\newcommand{\permusp}[1]{\mathcal{S}_{#1}}
\newcommand{\bigO}[1]{O\left(#1\right)}
\newcommand*{\rotmat}{\mathcal{R}}


%%%% MIXTURE FOR A PRIOR %%%%
\newcommand*{\hkmixtwgt}[1]{\alpha_{#1}}

%%%% MIXTURE OF EXPERTS %%%%
\newcommand*{\mixnum}{D}	% Number of components
\newcommand*{\mixvar}[2][]{\boldsymbol{\Upsigma}_{#2} \optexp{#1}}	% variance matrices
\newcommand*{\mixwgt}[2][]{\alpha_{#2}\optexp{#1}}	% weights
\newcommand*{\mixwgtvec}[1][]{\boldsymbol\alpha\optexp{#1}}
\newcommand*{\mixwgtspace}[1]{\mathcal{W}(#1)}
\newcommand*{\mixmeanf}{f}						% mean function
%\newcommand*{\mixmean}[2][]{\mathbf{m}_{#2}\optexp{#1}}		% means
\newcommand*{\mixmean}[2][]{\boldsymbol{\mu}_{#2}\optexp{#1}}
\newcommand*{\mixmeanvec}[1][]{\boldsymbol M\optexp{#1}}
\newcommand*{\mixvarvec}[1][]{\boldsymbol\Sigma\optexp{#1}}
\newcommand*{\mixbeta}[1]{\boldsymbol\beta_{#1}}	% parameters in the logistic regression
\newcommand*{\mixbetavec}[1][]{\underline{\boldsymbol\beta}\optexp{#1}}
\newcommand*{\mixbetavecsp}{\mathbb{B}}
%\newcommand*{\mixparamvec}[1][]{\boldsymbol\theta\optexp{#1}} % Whole vector of parameters
\newcommand*{\mixparamopt}{\mixparamvec^{N,\ast}}	% Optimal parameter
\newcommand*{\mixparamvecell}{\mixparamvec^{\ell}} % Required without optional arguments sometimes for LATEX reasons
\newcommand*{\mixparamvecellm}{\mixparamvec^{\ell-1}} % Required without optional arguments sometimes for LATEX reasons
\newcommand*{\mixparamsp}{\Theta} % Whole vector of parameters
%\newcommand*{\mixwgtcond}[4]{\completelike{#1}\left( #2 \middle| #3,#4 \right)} % 
\newcommand*{\mixwgtcond}[4]{\completelike{#1}(#2 | #3, #4)} %Conditional weights
\newcommand*{\suffstat}{\mathbf{s}} % Sufficient statistics
\newcommand*{\suffstatvec}{\boldsymbol S} % Sufficient statistics
\newcommand*{\mixsuffstat}[3]{\tilde S_{#1,#2}(#3)} % Sufficient statistics #2 for component #1
%\newcommand*{\mixsuffstat}[2]{\tilde S^{(#1)}_{#2}} % Alternative
\newcommand*{\mixsuffstatvec}{\boldsymbol {\tilde S}} % Sufficient statistics
\newcommand*{\ismixsuffstat}[3][]{\hat S_{#2,#3}\optexp{#1}} % Sufficient statistics #2 for component #1

\newcommand*{\mixk}[3][j]{\mixkfull{#2}{#3}{\mixmean{#1}}{\mixvar{#1}}}	% Component of the mixture
\newcommand*{\mixkfull}[5][]{r\optsub{#1}\left(#2,#3;#4,#5\right)}				% Full component

%%%% MULTIVARITATE T STUDENT DISTRIBUTIONS %%%%
\newcommand*{\tdens}[5][]{t\optsub{#1}(#2; #3, #4, #5)}
\newcommand*{\gammadens}[3]{\gamma\left(#1; #2, #3\right)}
\newcommand*{\df}{\nu}
\newcommand{\meanuu}{\frac{\df + \dimosptd}{\df + \mahalanobis{\pprva}{\mixmean{j}\prmat \partiextd{I}}{\mixvar{j}}}}
	% Conditional mean of uu (dirty hack to shorten notations)

%%%% TRICK FOR OVERLAPPING MATHS %%%
% For comparison, the existing overlap macros:
% \def\llap#1{\hbox to 0pt{\hss#1}}
% \def\rlap#1{\hbox to 0pt{#1\hss}}
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{%
\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{%
\rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{%
\clap{$\mathsurround=0pt#1{#2}$}}

% Stochastic independance in math mode
\catcode`\@=11
\def\indep{\setbox0\hbox{$\m@th\perp$}\mathrel{\hbox
         to1.25\wd0{\copy0\hss\box0}}}
\def\indep{\setbox0\hbox{$\m@th\perp$}\ifmmode\mathrel\fi{\hbox
         to1.25\wd0{\copy0\hss\box0}}}
\catcode`\@=12

%%%%%%% GROWTH MODEL %%%%%%%%%%
% PILOT \newcommand*{\bibound}{B}

